Text-DIAE: A Self-Supervised Degradation Invariant Autoencoders for Text Recognition and Document Enhancement

In this paper, we propose a Text-Degradation Invariant Auto Encoder (Text-DIAE), a self-supervised model designed to tackle two tasks, text recognition (handwritten or scene-text) and document image enhancement. We start by employing a transformer-based architecture that incorporates three pretext tasks as learning objectives to be optimized during pre-training without the usage of labeled data. Each of the pretext objectives is specifically tailored for the final downstream tasks. We conduct several ablation experiments that confirm the design choice of the selected pretext tasks. Importantly, the proposed model does not exhibit limitations of previous state-of-the-art methods based on contrastive losses, while at the same time requiring substantially fewer data samples to converge. Finally, we demonstrate that our method surpasses the state-of-the-art in existing supervised and self-supervised settings in handwritten and scene text recognition and document image enhancement. Our code and trained models will be made publicly available at~\url{ http://Upon_Acceptance}.

==> tables/ablation_loss_enhance.tex <==
% \begin{table}[t]
% \begin{tabular}{cc}
% % \caption{Ablation study of our model on DIBCO 2018 by removing different pre-training objectives}
% \label{tab:ablation_enhance}
% % \hline
% Method                     & PSNR  \\ \hline
% w/o pre-training           & -     \\
% w/o masking                & 18.59 \\
% w/o deblurring             & 18.70 \\
% w/o masking and deblurring & 19.06 \\ \hline
% full model                 & 19.18 \\ \hline
% \end{tabular}
% \end{table}
% \setlength{\tabcolsep}{2pt}
% \begin{table}[t]
% \scriptsize
% \centering
% \caption{Ablation study of our model on DIBCO 2018 by removing different pre-training objectives}
% \label{tab:ablation_enhance_objectives}
% \begin{tabular}{ll}
% \hline
% Method       & PSNR  \\ \hline
% w/o pre-training & 18.03 \\
% Pretraining w/o masking   & 18.59 \\
% Pretraining w/o deblurring       & 18.70 \\
% Pretraining w/o masking and deblurring      & 19.06 \\
% \textbf{full model}         & \textbf{19.18} \\ \hline
% \end{tabular}
% \end{table}
% \setlength{\tabcolsep}{1.4pt}

\begin{table}[t]
\begin{tabular}{llll}
\hline
$\mathcal{L}_{mask}$ & $\mathcal{L}_{blur}$ & $\mathcal{L}_{noise}$ & PSNR  \\ \hline
\xmark   & \xmark   & \xmark    & 18.75 \\
\xmark   & \cmark  & \cmark   & 19.34 \\
\cmark  & \xmark   & \cmark   & 19.45 \\
\xmark   & \xmark   & \cmark   & 19.82 \\
\cmark  & \cmark  & \cmark   & \textbf{19.95} \\ \hline
\end{tabular}
\end{table}



==> tables/ablation_loss_htr_str.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[t]
\scriptsize
\centering
\caption{\textbf{Ablations of the degradations as pre-training objectives.} Results in handwritten and scene-text recognition obtained by each pretext task. The performance is measured in terms of Word and Character error rates (WER and CER).}
\label{tab:ablation_htr_objectives}
\begin{tabular}{ccccccccc}
\hline\noalign{\smallskip}
\multirow{2}{*}{$\mathcal{L}_{mask}$} & \multirow{2}{*}{$\mathcal{L}_{blur}$} & \multirow{2}{*}{$\mathcal{L}_{noise}$} & \multicolumn{3}{c}{IAM}& \multicolumn{3}{c}{IC13}\\
& & & CER & WER & Average &CER & WER & Average \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
%\xmark &\xmark&\xmark& 11.8 & 31.3 & 21.55 \\
\cmark &\xmark&\xmark& \textbf{7.5}	&\textbf{19.9}	&\textbf{13.7} & 3.4 & 8.0 & 5.7 \\
\cmark &\cmark&\xmark& 9.9	&24.8	&17.3 & \textbf{3.2}	& \textbf{8.0} &	\textbf{5.6} \\
\cmark &\xmark&\cmark& 9.0	&23.3	&16.1& 3.7&	8.6	&6.2 \\
\cmark &\cmark&\cmark& 9.3	&23.8 &	16.6 & 4.0&	9.3	&6.7 \\
\hline
\end{tabular}
\end{table}
\setlength{\tabcolsep}{1.4pt}


% \setlength{\tabcolsep}{2pt}
% \begin{table}[t]
% \scriptsize
% \centering
% \caption{Ablation study of our model on IAM dataset by removing different pre-training objectives}
% \label{tab:ablation_htr_objectives}
% \begin{tabular}{cccccc}
% \hline\noalign{\smallskip}
% $\mathcal{L}_{mask}$ & $\mathcal{L}_{blur}$ & $\mathcal{L}_{noise}$ &CER & WER & Average \\
% \noalign{\smallskip}
% \hline
% \noalign{\smallskip}
% %\xmark &\xmark&\xmark& 11.8 & 31.3 & 21.55 \\
% \cmark &\xmark&\xmark& {21.2} & \textbf{50.5} & {35.8} \\
% \cmark &\cmark&\xmark& \textbf{20.3} & 50.6 & \textbf{35.4} \\
% \cmark &\xmark&\cmark& 23.1 & 54.6 & 38.8 \\
% \cmark &\cmark&\cmark& 25.3 & 58.9 & 42.2 \\
% \hline
% \end{tabular}
% \end{table}
% \setlength{\tabcolsep}{1.4pt}

==> tables/ablation_loss_str.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[t]
\scriptsize
\centering
\caption{Ablation study of our model on IAM dataset by removing different pre-training objectives}
\label{tab:ablation_htr_objectives}
\begin{tabular}{cccccc}
\hline\noalign{\smallskip}
$\mathcal{L}_{mask}$ & $\mathcal{L}_{blur}$ & $\mathcal{L}_{noise}$ &CER & WER & Average \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
%\xmark &\xmark&\xmark& 11.8 & 31.3 & 21.55 \\
\cmark &\xmark&\xmark& {21.2} & \textbf{50.5} & {35.8} \\
\cmark &\cmark&\xmark& \textbf{20.3} & 50.6 & \textbf{35.4} \\
\cmark &\xmark&\cmark& 23.1 & 54.6 & 38.8 \\
\cmark &\cmark&\cmark& 25.3 & 58.9 & 42.2 \\
\hline
\end{tabular}
\end{table}
\setlength{\tabcolsep}{1.4pt}

==> tables/binarization_table.tex <==
% \begin{figure}[t]
%   \begin{center}
%   \label{tab:binarization_qualitative}
%   \footnotesize
%   \renewcommand{\arraystretch}{0.5} 
%   \begin{tabular}{ccc}
 
%     \includegraphics[width=0.3 \columnwidth, height=20mm]{images/comparison_DIE_2017/3_deg_17.png} &
%     \includegraphics[width=0.3 \columnwidth, height=20mm]{images/comparison_DIE_2017/3_gt_17.png}&
%     \includegraphics[width=0.3 \columnwidth, height=20mm]{images/comparison_DIE_2017/sauvola.png}\\ 
    
    
%     % \noalign{\smallskip}
%     Original  & Ground Truth & Sauvola et. al.~\cite{sauvola2000adaptive}
%     % \vspace{-0.2cm}
%     \\ %\noalign{\smallskip}     
    
%     \includegraphics[width=0.3 \columnwidth, height=20mm]{images/comparison_DIE_2017/kang.png}&
%     \includegraphics[width=0.3 \columnwidth, height=20mm]{images/comparison_DIE_2017/docentr.png}&
%     \includegraphics[width=0.3 \columnwidth, height=20mm]{images/comparison_DIE_2017/3_pred.png}
%     \\%\noalign{\smallskip}   
%     Kang et al.~\cite{kang2021complex}& DocEnTr~\cite{souibgui2022docentr} & \textbf{Text-DIAE}
%     \\%\noalign{\smallskip}   

%     \end{tabular}
%   \end{center}
%   \caption{\textbf{Binarization Results} We show the results of the binarization task. Given an input degraded image, our model performs significantly better qualitatively compared to previous approaches.}
% \end{figure}

==> tables/deblurring_table.tex <==
% \begin{table}[t]
% \caption{Comparitive results on document deblurring }
% \label{tab:deblur_results}

% \begin{tabular}{@{}ll@{}}
% \toprule
% Method       & PSNR  \\ \midrule
% CNN-Baseline & 19.36 \\
% Pix2Pix-HD   & 19.89 \\
% DE-GAN       & 20.37 \\
% DocEnTr      & 21.28 \\
% DIAE         & 23.58 \\ \bottomrule
% \end{tabular}%

% \end{table}
\setlength{\tabcolsep}{2pt}
\begin{table}[t]
\scriptsize
\centering
\caption{Comparitive results on document deblurring}
\label{tab:deblur_results}
\begin{tabular}{ll}
\hline
Method       & PSNR  \\ \hline
CNN-Baseline~\cite{hradivs2015convolutional} & 19.36 \\
Pix2Pix-HD~\cite{wang2018high}   & 19.89 \\
DE-GAN~\cite{souibgui2020gan}       & 20.37 \\
DocEnTr~\cite{souibgui2022docentr}      & 21.28 \\
\textbf{Ours}         & \textbf{23.58} \\ \hline
\end{tabular}
\end{table}
\setlength{\tabcolsep}{1.4pt}


==> tables/finetuning_iam.tex <==

% \begin{minipage}{.35\textwidth}

\setlength{\tabcolsep}{2pt}

\begin{table}[t]
\scriptsize
% \footnotesize
\begin{center}
\caption{\textbf{SOTA results.} Word and character error rates (WER and CER) of the proposed method compared to current state-of-the-art methods on the IAM word level dataset.}
\label{table:results_fine_tuning_iam}
\begin{tabular}{lccc}
\hline\noalign{\smallskip}
Method & WER & CER & Average \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
Bluche et al. \cite{bluche2015deep}  & 24.7 & \textbf{7.3}& 16.00 \\
Bluche et al. \cite{bluche2016joint} & 24.6 & 7.9 & 16.25 \\
Sueiras et al.  \cite{sueiras2018offline}& 23.8 & 8.8 & 16.30 \\
ScrabbleGAN \cite{fogel2020scrabblegan} & 23.6 & - & - \\
SSDAN \cite{zhang2019sequence} & 22.2 & 8.5 & 15.35 \\
SeqCLR \cite{aberdam2021sequence} & 20.1 & 9.5 & 14.80 \\
Ours & \textbf{19.9} & 7.5 & \textbf{13.70} \\
% Ours-Large & & & \\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

% \end{minipage}

==> tables/qualitative_samples_ocr.tex <==
\setlength{\extrarowheight}{20pt}
\newcommand{\centered}[1]{\begin{tabular}{c} #1 \end{tabular}}
% >{\centering\arraybackslash}
\begin{table}[h]
\caption{\textbf{OCR predictions after deblurring} Comparison of deblurring methods and OCR predictions (Tesseract) on top the results with CER. 
% We use the OCR performance with the Character Error Rate (CER). Our proposed method (DIAE) outputs an image that is more suitable to be used as input to an OCR system. We decrease considerably the CER, 10,57 difference, compared to the previous best performing approach. 
The first column (Deg.) stands for Degradation type. Text in red are OCR mistaken predictions.}
\label{tab:blur_qualitative}
\tiny
\centering
% \begin{center}
\begin{tabular}{>{\centering\arraybackslash} m{0.5cm}|>{\centering\arraybackslash} m{4cm}|>{\centering\arraybackslash} m{1.5cm}| >{\centering\arraybackslash} m{4.5cm}|>{\centering\arraybackslash} m{.5cm}}
\hline
\textbf{Deg.}& \textbf{Image} & \textbf{Source} & \textbf{OCR} & \textbf{CER} \\ \hline

\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Blur}}} & \includegraphics[width=26mm, height=10mm]{images/qualitative_samples_ocr/blur_orig.png}
& Orig & "\textcolor{red}{Mae yw spaniedod' i}f \textcolor{red}{MA APAIMAAPEdosh an}elf, 
\textcolor{red}{Awanaisnn A d}n\textcolor{red}{nmoupi}l \textcolor{red}{1 Mie Myrtle dial cell }s\textcolor{red}{agos Alo Wie sascled saesye dias,}" & 78.86 \\ \cline{2-5} 
 & 
 \includegraphics[width=26mm, height=10mm]{images/qualitative_samples_ocr/blur_gt.png}
 & GT & "the parameters of the common del itself, because it necessarily r the hypothetical wealth shares ndeed the model were true\textcolor{red}{:}" & 4.88 \\ \cline{2-5} 
 & 
 \includegraphics[width=26mm, height=10mm]{images/qualitative_samples_ocr/blur_docentr.png}
 & DocEnTr\cite{souibgui2022docentr} & "the parameters of\textcolor{red}{Ur}e co\textcolor{red}{n}m\textcolor{red}{nn}on del it\textcolor{red}{ic}if, because it \textcolor{red}{m}ece\textcolor{red}{n}sar\textcolor{red}{t}ly r the hypot\textcolor{red}{ic}tical wealth shares nd\textcolor{red}{o}ed the modal w\textcolor{red}{o}r\textcolor{red}{n} tru\textcolor{red}{c}." & 19.51 \\ \cline{2-5} 
 &
 \includegraphics[width=26mm, height=10mm]{images/qualitative_samples_ocr/blur_pred.png}
 & Ours &"te parameters of the common del it\textcolor{red}{u}elf, because i necessari\textcolor{red}{t} r the hypothetical wealth shares \textcolor{red}{r}deed the model were true." & \textbf{8.94} \\ \hline
% \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Noise}}} 
% & 
%  \includegraphics[width=45mm, height=12mm]{images/qualitative_samples_ocr/another_orig.png}
% & Orig &"I any thingobfcure,notunderftood,,., ... , Be here, the State expounds the darkeft wood: And makes the thickeft thickets p!ain-and clear," & 17.97 \\ \cline{2-5} 
%  & 
%   \includegraphics[width=45mm, height=10mm]{images/qualitative_samples_ocr/another_gt.png}
%  & GT &"J F any thing obfcure, not underftood Be here, the State expounds the darkeft wood:And makes the thickeft thickets p!ain and clear," & 10.94 \\ \cline{2-5} 
%  & 
%   \includegraphics[width=45mm, height=10mm]{images/qualitative_samples_ocr/another_docentr.png}
%  & DocEnTr &"F any thing obfcure, not underftoodBe here, the State exposnds the darkeft wood: Aod makes che thickeft thickets p!tin and clear" & 13.28 \\ \cline{2-5} 
%  & 
%   \includegraphics[width=45mm, height=10mm]{images/qualitative_samples_ocr/another_pred.png}
%  & DIAE &ji any thing obfcure, not underftood Be here, the State expounds the darke ft wood: And makes che thickeft thickets p!tin and clear," & 12.50 \\ \hline

\end{tabular}
\end{table}




